Spatio-Temporal Multi-Subgraph GCN for 3D Human Motion Prediction

Human motion prediction (HMP) involves forecasting future human motion based on historical data. Graph Convolutional Networks (GCNs) have garnered widespread attention in this field for their proficiency in capturing relationships among joints in human motion. However, existing GCN-based methods tend to focus on either temporal-domain or spatial-domain features, or they combine spatio-temporal features without fully leveraging the complementarity and cross-dependency of these two features. In this paper, we propose the Spatial-Temporal Multi-Subgraph Graph Convolutional Network (STMS-GCN) to capture complex spatio-temporal dependencies in human motion. Specifically, we decouple the modeling of temporal and spatial dependencies, enabling cross-domain knowledge transfer at multiple scales through a spatio-temporal information consistency constraint mechanism. Besides, we utilize multiple subgraphs to extract richer motion information and enhance the learning associations of diverse subgraphs through a homogeneous information constraint mechanism. Extensive experiments on the standard HMP benchmarks demonstrate the superiority of our method.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> mainbody/2.related.tex <==
\section{Related Work}
\label{sec:related}
% \textbf{Human motion prediction.} 
% % Early methods for human motion prediction captured shallow temporal dynamics using state prediction, such as the Hidden Markov Model~\cite{lehrmann2014efficient,liu2017human,mathew2012predicting},  Gaussian process latent variable models~\cite{wang2005gaussian}, and Restricted Boltzmann Machines~\cite{starke2019neural}. However, these methods struggle to model the complex dynamics of human motion and require substantial feature engineering for accurate predictions.
% Recent advancements in deep learning have significantly improved human motion prediction by enabling the learning of complex spatio-temporal representations. RNN-based models like ERD~\cite{fragkiadaki2015recurrent}, Structural-RNN~\cite{jain2016structural}, Res-sup~\cite{martinez2017human} and AHMR~\cite{liu2022investigating} have enhanced temporal dependency modeling. 
% CNNs~\cite{li2018convolutional,cui2021efficient} excels at capturing spatial information. Furthermore, Long Short-Term Memory Networks~\cite{yuan2019ego,lee2021video}, and Transformer Networks~\cite{cai2020learning,aksan2021spatio,martinez2021pose} have demonstrated promising results in learning rich representations from motion sequences, leading to more accurate predictions.
% In contrast to the aforementioned methodologies, our focus lies in exploring the application of GCN to better understand complex spatio-temporal dependencies in human motion, resulting in more precise predictions.

\textbf{Human motion prediction.}%Spatio-temporal Representation
Current research primarily focuses on improving the model or designing spatio-temporal feature extraction methods~\cite{ma2022progressively,li2022skeleton,xu2023eqmotion,zhang2023dynamic}. They commonly extract features from the frequency space and use the Discrete Cosine Transform (DCT) as a routine operation in the data preprocessing stage. Although DCT can model the time dependency of each joint node well, it tends to ignore the constraint relationships between joint nodes. While GCNs have partly alleviated this issue, existing GCN-based models often overlook the interactions between spatio-temporal features~\cite{aksan2021spatio,li2022skeleton,ma2022progressively,zhong2022spatio}. 
Differently, our method leverages the complementary nature of spatio-temporal information across multiple scales during the process of  modeling the temporal smoothness and spatial dependencies among human motion.

\noindent \textbf{Design of Graph Convolution Networks.} 
% Recent advances in HMP have prominently centered on GCN, which adeptly captures both temporal and spatial dependencies.
Researchers have explored diverse graph structures in GCN to encode skeleton connections and prior knowledge.
\cite{sofianos2021space} extends graph convolution to model both temporal and spatial dependencies, while \cite{li2022skeleton} proposes graph scattering networks to decompose pose features. To address challenges from incomplete observations, \cite{feichtenhofer2022masked} pioneers a multi-task GCN. \cite{zhong2022spatio} proposed a gating-adjacency GCN to extract spatio-temporal information and fuse those information with the Kronecker product.
Differently, our method employs diverse subgraphs to enhance the model's understanding of human behavior, coupled with a homogeneous information constraint mechanism that strengthens associations among subgraphs.  
% This refinement yields an improved understanding of motion variations across different types, thereby elevating the model's overall performance.
% This approach improves the model’s ability to capture motion variations, leading to enhanced overall performance.


==> mainbody/rebuttal.tex <==
\newpage

We appreciate all reviewers for their efforts and time.
Your valuable comments greatly improved the quality of our
paper. Next, we will reply to each reviewer separately.

\textcolor{blue}{\textbf{To Reviewer $\#1$.}} 
We sincerely appreciate your recognition of our work. 
Your acknowledgment of the novelty, clarity, and rigorous experimental validation in our study motivates us to continue contributing meaningful insights to the community. Thank you again for your valuable feedback and support.

\textbf{\textcolor{magenta}{To Reviewer $\#2$.}}
% A more explicit description of how the multi-subgraph GCN architecture improves predictive performance might enhance the paper.
\textbf{Q1: More description of the multi-subgraph GCN architecture.}
Thank you for your valuable feedback. The multi-subgraph GCN architecture enables the model to capture a broader range of motion patterns. 
While the GCN follows standard architecture principles without special designs, each subgraph offers unique insights into shared motion patterns, effectively capturing the motion characteristics. Besides, the homogeneous information constraint enhances the complementary relationship between subgraphs, further improving the model's capacity to represent and predict human motion accurately. We will include these clarifications in the revised version.
%The loss function is well-defined, but it might be helpful to provide more context on how the hyperparameter λ is chosen or tuned.
\textbf{Q2: More context about $\lambda$.}
Thank you for pointing this out. We selected the hyperparameter $\lambda$ through systematic tuning, as detailed in Fig.~\ref{table:lambda} of the manuscript. Specifically, we explored a range of values $\{0, 10^{-3}, 10^{-2}, 10^{-1}, 1\}$ and evaluated their effect on model performance. The results indicate that $\lambda$ = 0.1 achieves the best balance between enforcing homogeneous information constraints and maintaining the flexibility of spatio-temporal branches, yielding the lowest MPJPE. This process provides clear guidance for choosing $\lambda$ in practical applications.
%The conclusion could briefly mention any future work or potential applications of the method to provide a broader perspective on the impact of the research.
%结论调整
\textbf{Q3: Conclusion.}
Thank you for your valuable suggestion. We have revised the conclusion to include potential future work and applications of our method, such as its extension to action recognition and pose estimation, thereby providing a broader perspective on the impact and applicability of our research.

\begin{table}[h]%\footnotesize|tiny
\renewcommand{\thetable}{1}
\centering
\setlength{\tabcolsep}{8pt} % 设置列间距为3.5pt 5
\caption{Comparison of different designs for $\widetilde{\mathbf{Y}}$ in H3.6M. ``Avg." represents $\widetilde{\mathbf{Y}}=\frac{1}{2}(\mathbf{Y}^{T,L}+\mathbf{Y}^{S,L})$.}
\label{tab:_st}
\begin{tabular}{l|cccccc}
\toprule 
$\widetilde{\mathbf{Y}}$ &80ms &160ms &320ms &400ms &Avg. \\ \hline
$\mathbf{Y}^{T,L}$ & 10.00 &22.21 &47.31 &58.58 &34.52\\
$\mathbf{Y}^{S,L}$ & \textcolor{red}{9.61} &\textcolor{red}{21.63} &\textcolor{red}{46.40} &\textcolor{red}{57.55} &\textcolor{red}{33.80} \\ 
Avg.& 9.71 &21.75 &46.63 &57.81 &33.98\\  
 \bottomrule
\end{tabular}
\end{table}

\textbf{\textcolor{cyan}{To Reviewer $\#4$.}}
%The difference between STMS-GCN and the separate models is not clear, as the separate models also fuse temporal and spatial information. Could you provide a clearer comparison with a formal theoretical analysis, rather than relying solely on figure comparison?
%d和C的优势对比：怎么混合是一个大问题
\textbf{Q1: The difference between STMS-GCN and the separate models.}
Thank you for your valuable comment. We have revised the manuscript to provide a clearer comparison between STMS-GCN and the separate models. Specifically, we highlight the following distinctions:  
\textbf{1) Fusion Mechanism}: Unlike the separate models that fuse temporal and spatial features only at the output stage, STMS-GCN proposes an interaction mechanism between temporal and spatial branches during intermediate feature learning. This allows for a more refined and complementary exchange of information across domains.  
In contrast,  simple fusion under the separate models can't fully exploit each branch's advantages, and effectively combining both branches' strengths is challenging. Results of using various outputs as the final result are shown in Tab.\ref{tab:_st}, indicating that utilizing the spatial branch's output (ours design) achieves the best.
\textbf{2) Cross-Domain Knowledge Distillation}: Our method leverages a spatio-temporal information interaction to reinforce cross-domain knowledge transfer, enabling better alignment of temporal and spatial representations. This is absent in separate models.  
%What is the core challenge addressed by your contributions? The cross-domain information contrast mechanism seems straightforward.
\textbf{Q2: Core challenge.}
The core challenge we address is effectively capturing the complementary nature of spatio-temporal dependencies in HMP. Existing methods often focus on individual domains or integrate spatio-temporal relationships by blending various convolutional kernels, which fail to capture the complex interactions and hidden cross-domain dependencies. Our cross-domain information contrast mechanism overcomes this by explicitly reinforcing the relationship between spatial and temporal branches, leading to more robust feature learning and improved generalization across diverse motion patterns, as shown by our superior performance in extensive experiments.
%The datasets used are unclear. Could you provide more details about the size and structure of the input datasets?
%数据集的使用不清晰
% H3.6M和CMU Mocap是该研究方向最常用的数据集，在具体实验中我们遵循常见的数据集使用方式，如Traj-GCN、SPGSN、STS-GCN，并未涉及到任何特殊处理。
\textbf{Q3: Datasets.}
The H3.6M and CMU-Mocap datasets are commonly used in this research domain. 
H3.6M consists of motion data of 11 actors performing 15 common actions.
Following the standard paradigm, we train the models on the segmented clips in the 6 subjects and test on the specific clips in the 5th subject.
CMU-Mocap contains motion capture data of various human activities and has been widely used in various applications. Following the evaluation protocol used in previous works, we evaluate the performance of 8 human action categories.
%In Table 1, why does your approach not achieve one of the top two best results in the 560ms column? What are the limitations of your approach, and in what scenarios does your method underperform compared to SOTA works?
%表1中我们方法在560ms表现不佳的原因
\textbf{Q4: Performance and limitations.}
Although our method does not achieve the top two results at 560ms in Table 1, it shows competitive performance. The slightly lower performance at 560ms can be attributed to our method's focus on capturing overall spatio-temporal dependencies, which may trade off some accuracy in short-term predictions. 
Regarding limitations, our method introduces a small computational overhead due to the interaction of diverse subgraphs. Additionally, it may also underperform in scenarios where motion patterns are highly erratic or lack clear temporal consistency, as such cases challenge the model’s ability to effectively distill cross-domain knowledge.
%The ablation study is not sufficiently detailed. It would be useful to clearly explain the improvement gained from each contribution, as the current statement is too superficial.
%消融实验的详细解释说明
\textbf{Q5: More explain about ablation study.}
Thank you for your suggestions. we will provided a more detailed ablation study, clearly outlining the contributions of each component and the corresponding performance improvements in the revised version.
% we have revised the corresponding section to explicitly analyze the contributions of each component of our method. Specifically, we conducted additional experiments to separately evaluate the impact of multi-subgraph learning, homogeneous information constraints, and cross-domain knowledge transfer mechanisms. The results, now detailed in the revised ablation study, clearly demonstrate the individual and cumulative improvements from these contributions, providing a more comprehensive understanding of their effectiveness.
% In Table 3, why does the best result at 80ms come from Gs+L1, rather than from the model that includes all methods?
%为什么80ms没有取得最佳。GS更多关注短期的，GS关注长期的，实验结果可以明显看到
\textbf{Q6: $\mathbf{G}_S + \mathbf{L}_1$.}
$\mathbf{G}_S + \mathbf{L}_1$ performs best at 80ms due to its simpler structure, which better captures short-term motion dynamics by avoiding potential interference from additional constraints or modules. However, for longer-term predictions, the full model demonstrates superior performance, because it better captures and utilizes complex spatio-temporal dependencies. This highlights the trade-off between model simplicity and capacity at different prediction horizons.
